Towards a Domain-Specific Modelling Environment for Reinforcement Learning

In recent years, machine learning technologies have gained immense popularity and are being used in a wide range of domains. However, due to the complexity associated with machine learning algorithms, it is a challenge to make it user-friendly, easy to understand and apply. Machine learning applications are especially challenging for users who do not have proficiency in this area. In this paper, we use model-driven engineering (MDE) methods and tools for developing a domain-specific modelling environment to contribute towards providing a solution for this problem. We targeted reinforcement learning from the machine learning domain, and evaluated the proposed language, reinforcement learning modelling language (RLML), with multiple applications. The tool supports syntax-directed editing, constraint checking, and automatic generation of code from RLML models. The environment also provides support for comparing results generated with multiple RL algorithms. With our proposed MDE approach, we were able to help in abstracting reinforcement learning technologies and improve the learning curve for RL users.

==> frozenlake.tex <==
\subsection{Frozen Lake Application}
    
The frozen lake application is a popular application in reinforcement learning problems \cite{Ravichandiran2018}. The agent here will learn to navigate in the frozen lake environment (see Fig. \ref{fig:FrozenLakeEnv}). avoiding what is called holes in the lake, because whenever the agent takes a step to a hole state, that will terminate the training episode, without reaching to the goal state, meaning the agent can not make any further actions from the hole states. %The RLML model for frozen lake application is presented in Fig.~\ref{fig:FrozenLakeRLML}.
    
    \begin{figure}[!tbh]
        \centering
        \includegraphics[width=0.5\linewidth]{images/FrozenLake/FrozenLakeEnv.png}
        \caption{Frozen Lake Environment}
        \label{fig:FrozenLakeEnv}
    \end{figure}

    For space reasons, we only present the result of the Q-learning algorithm on this application here (see Fig. \ref{fig:FrozenLakeResult}). Studying the \emph{Q-Table} and policy values we notice that the agent successfully learned to navigate the frozen lake environment and avoided any hole state. In the policy table, none of the states take an action to go to state H, except when the initial state starts from H, which will end the navigation and in turn the training episode.
   
    \begin{figure}[!tbh]
        \centering
        \includegraphics[width=\linewidth]{images/FrozenLakeEnvInputVals.png}
        \caption{Frozen Lake: Input Values for Environment}
        \label{fig:FrozenLakeEnvInputVals}
    \end{figure}
    
    \begin{figure}[!tbh]
        \centering
        \includegraphics[width=0.8\linewidth]{images/FrozenLake/FrozenLakeResult_v2.png}
        \caption{Frozen Lake: Q-Learning Result}
        \label{fig:FrozenLakeResult}
    \end{figure}

    For more details on the use of RLML on the frozen lake application, please refer to \cite{boudakian-mrp-2022}. The artifacts are available at \url{https://github.com/mde-tmu/RLML}.
    



